SGC-VQGAN: Towards Complex Scene Representation via Semantic Guided Clustering Codebook

Vector quantization (VQ) is a method for deterministically learning features through discrete codebook representations. Recent works have utilized visual tokenizers to discretize visual regions for self-supervised representation learning. However, a notable limitation of these tokenizers is lack of semantics, as they are derived solely from the pretext task of reconstructing raw image pixels in an auto-encoder paradigm. Additionally, issues like imbalanced codebook distribution and codebook collapse can adversely impact performance due to inefficient codebook utilization. To address these challenges, We introduce SGC-VQGAN through Semantic Online Clustering method to enhance token semantics through Consistent Semantic Learning. Utilizing inference results from segmentation model , our approach constructs a temporospatially consistent semantic codebook, addressing issues of codebook collapse and imbalanced token semantics. Our proposed Pyramid Feature Learning pipeline integrates multi-level features to capture both image details and semantics simultaneously. As a result, SGC-VQGAN achieves SOTA performance in both reconstruction quality and various downstream tasks. Its simplicity, requiring no additional parameter learning, enables its direct application in downstream tasks, presenting significant potential.

==> tables/category.tex <==
\begin{table}[t]
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c}
\hline
0 & fish & 8 & food & 16 & natural landscape\\
1 & other small sea creatures & 9 & small beasts & 17 & little stuff\\
2 & other large sea creatures & 10 & dogs & 18 & medium stuff\\
3 & birds & 11 & great beasts & 19 & plants\\
4 & small terrestrial animals & 12 & medium beasts & 20 & clothing\\
5 & insects & 13 & vehicles & 21 & musical instruments\\
6 & vegetables& 14 & buildings & 22 & furnitures\\
7 & fruits & 15 & public facilities & 23 & people\\
\hline

\end{tabular}
}
\caption{The merged categories and corresponding semantic categories mask feature map pixel values based on the original 919 categories.}
\label{tab:imgnt_lei}
\end{table}
